Leveraging Sparse Linear Layers for Debuggable Deep Networks

We show how fitting sparse linear models over learned deep feature representations can lead to more debuggable neural networks. These networks remain highly accurate while also being more amenable to human interpretation, as we demonstrate quantiatively via numerical and human experiments. We further illustrate how the resulting sparse explanations can help to identify spurious correlations, explain misclassifications, and diagnose model biases in vision and language tasks. The code for our toolkit can be found at https://github.com/madrylab/debuggabledeepnetworks.

==> intro_alt.tex <==
\section{Introduction}


%We plan to release our solver and toolkit.

%%%%%%%%% Eric's intro %%%%%%%%%%%
As deep networks continue to improve and be applied to a variety of 
tasks, researchers are increasingly scrutinizing the inner workings and 
learned behaviors of these models. For both legal and practical reasons, 
recent works have probed deep networks over a range topics in order to 
diagnose various potential shortcomings and understand their behavior. 
For example, gender classification systems have been found to be biased 
against darker-skinned females \citep{buolamwini2018gender}, while 
toxic comment classification systems were later identified to be biased 
against identity groups \citep{zorian2019debiasing}. Image recognition 
systems were found 
to be depending on spurious correlations, capable of 
identifying cows in pastures but not on beaches \citep{beery2018recognition}, 
or relying on 
visual artifacts for skin-lesion classification \citep{bissoto2020debiasing}. 
At the same time, business and corporations are under legal pressure 
to provide explanations for deep network predictions, such as to explaining  
the process behind assigning credit scores to satisfy regulations \citep{} 
and satisfying general data protection regulations \citep{}. 

One way of gaining insight into these problems is to first understand 
what concepts a deep network has learned by interpreting the individual  
hidden units (neurons) within the model. This task has been the focus of 
an extensive line of work known as feature interpretation 
methods, for example by visualizing 
neurons~\citep{yosinski2015understanding} 
or assigning labels to neurons~\citep{bau2017network}. 
Although these methods can shed light on the types of inputs that activate 
specific neurons, using this knowledge to diagnose general behaviors 
or properties of a 
deep network can still be quite challenging for modern deep architectures. 
This is primarily due to the sheer scale of deep networks: 
even at the final hidden layer, there are simply far too many neurons
and parameters for a practitioner to feasibly interpret, which can easily 
exceed thousands of neurons and millions of parameters.  
% These methods range from fitting a simpler, interpretable models as a 
% local proxy~\citep{ribeiro2016should} to constructing saliency
% maps~\citep{simonyan2013deep} or 
% counterfactuals~\citep{goyal2019counterfactual}. 
% However, by design, these explanations can only yield a highly local 
% snapshot of 
% the model's decision making process, and some work has questioned 
% whether the resulting explanations are faithful to the model or causally 
% linked to the model's prediction~\citep{adebayo2018sanity}. 
% While both of these types of methods can excel at generating explanations 
% for specific 
% neurons or specific examples, it is not always obvious how they can be 
% effectively 
% used to identify and debug global patterns that a deep network learns, 
% such as correlations and biases.

In order to simplify this problem, we study a natural approach of 
sparsifying 
the final linear layer of the deep neural network.  
By greatly reducing the number of features, the feature interpretation 
methods 
become more viable to humans for diagnosing underlying properties of 
deep networks. 
At the same time, we can continue to leverage the expressive power of the 
deep 
representation, allowing the sparse linear layer to maintain 
much of the original performance. 
Although simple in concept, we find that our approach allows us to develop 
a 
deeper understanding of the internal reasoning process of modern, 
complex 
architectures, without having to manually inspect an overwhelming number 
of examples or neurons. 

We demonstrate the approach in several case studies covering typical 
architectures used in a range of vision and language classification tasks. 
In the vision domain, we analyze residual architectures for the Places 
\citep{} 
and ImageNet \citep{} datasets, where we find that the sparse linear model 
allows us to more easily identify (possibly spurious) correlations between 
classes, 
as well as provide explanations for misclassifications. We corroborate these 
findings with additional human-in-the-loop experiments via Amazon Turk, 
where we 
find that humans are more accurate at guessing the model prediction when 
shown 
features from the sparse linear model over the dense linear model. 
In the language domain, we analyze BERT-based architectures for 
sentiment 
classification \citep{} and toxic comment classification \citep{}, where we 
find 
that our approach allows us to identify strong keywords which can be used 
to construct
sentiment counterfactuals and identify unintended biases for (or against) 
particular identities. 
We also develop a visualization technique for interpreting the neurons of a 
language model via word clouds. Finally, we have released our open-source 
solver 
for efficiently computing elastic net regularization paths on large-scale 
datasets (i.e. ImageNet) that cannot be fitted with existing solvers, which 
may find use in problems beyond interpretability when fitting sparse linear 
models. 
\eric{update as we finalize experiments to show}

% \paragraph{Our contributions}
% \begin{itemize}
% 	\item We demonstrate in a number of case studies how sparsifying the final 
% 	linear can aid in diagnosing underlying properties of a deep network. These 
% 	diagnostics range from uncovering correlations and biases used in ImageNet 
% 	classifiers or BERT based language models, to providing explainations for 
% 	misclassifications and generating counterfactuals. 
% 	\item We evaluate how sparsity of the linear classifiers can improve 
% 	the ability of a human to understand how the network makes prediction, 
% 	via human-in-the-loop experiments using Amazon Turk. 
% 	\eric{update after shibani pushes update to mturk}
% 	\item In order to fit the sparse linear models, we have implemented a 
% 	SAGA-based solver for efficiently computing elastic net regularization paths on 
% 	large-scale datasets (i.e. ImageNet size) which cannot be fitted with 
% 	existing solvers. Our implementation is open-source and widely applicable 
% 	to fitting sparse linear models for large-scale problems beyond 
% 	interpretability. 
% \end{itemize}



% Despite their widespread usage and impressive performance, a long-standing criticism 
% of deep neural networks is their black-box, inexplainable nature. 
% Although large-scale modern architectures such as 
% transformers~\citep{brown2020language} and deep residual networks~\citep{tan2019efficientnet} 
% can achieve impressive, state-of-the-art performance, 
% explaining their underlying decision processes remains a herculean task. 
% However, interpretability is a prerequisite in many real-world settings, 
% including high-stakes applications such as 
% medicine~\citep{azodi2020opening,hendriks2020machine} and  
% criminal 
% justice~\citep{TODO}, human-ML collaboration scenarios~\citep{TODO}, 
% or meeting new legal requirements \citep{barocas2020hidden}. 
% The pressure to develop interpretable deep learning systems is further 
% compounded by rising ethical concerns on the biases learnt by these 
% systems~\citep{buolamwini2018gender}.

% These questions have been the focus of an extensive line of work 
% which aims to define and satisfy meaningful notions of interpretability 
% for deep networks.
% One class of methods, known as feature interpretation 
% methods~\citep{yosinski2015understanding,bau2017network}, 
% focuses on understanding \emph{what} individual units (neurons) within a deep 
% network correspond to.
% Although these methods can shed light on the types of inputs that activate 
% specific neurons, using these neurons to reason about a network's prediction
% is challenging due to the sheer number and redundancy of hidden units. 
% In contrast, feature attribution methods aim to explain \emph{why} a network  
% made a certain prediction for a specific input. 
% These methods range from fitting a simpler, interpretable models as a 
% local proxy~\citep{ribeiro2016should} to constructing saliency
%  maps~\citep{simonyan2013deep} or counterfactuals~\citep{goyal2019counterfactual}. 
% However, by design, these explanations can only yield a highly local snapshot of 
% the model's decision making process, and some work has questioned 
% whether the resulting explanations are faithful to the model or causally 
% linked to the model's prediction~\citep{adebayo2018sanity}. 
% While both of these types of methods can excel at generating explanations for specific 
% neurons or specific examples, it is not always obvious how they can be effectively 
% used to identify and debug global patterns that a deep network learns, 
% such as correlations and biases.  

% Eric: This paragraph was pretty redundant to the proceeding paragraph, 
% and so I merged them together. I left the original two here, but commented out

% In this work, we take an alternative approach, focusing instead 
% on the simpler problem of interpreting a deep network as a linear model applied to a
% deep feature representation. 
% This task can be highly non-trivial for typical modern deep networks, 
% whose final linear classifiers have up to thousands of (learned) input features 
% and millions of parameters. 
% To alleviate this problem, our strategy is to 
% optimally replace the \emph{dense} linear layer of a given deep 
% network with a \emph{sparse} one.
% The resulting model maintains performance comparable to the original deep network, 
% but with predictions that can be fully explained with a small number of linear operations 
% on a concise set of deep features. 
% Our approach allows us to take a step towards combining the interpretability of 
% simpler linear models with the performance of deep networks.


% At a high-level, our approach is to decompose a given
% deep network into a deep representation followed by a \emph{sparse} linear 
% model (cf. Figure~\ref{fig:decomposition}). 
% We can then leverage the strengths of existing interpretability techniques: a 
% naturally interpretable linear model~\cite{studies} explains how the network 
% makes its decisions 
% based on a sparse set of features, which in turn, can be understood using 
% standard feature interpretation methods.  
% \eric{rethink end to end phrasing here}
% \eric{a) what about this isn't end to end? b) not so sure about the causal again}
% While our approach tackles a seemingly simpler problem than end-to-end 
% interpretability, it allows us to develop a causal understanding into the internal 
% reasoning process of the model.
% In fact, we show that explanations based on this approach serve as a powerful 
% tool to debug state-of-the-art deep networks, both at the global level (e.g., 
% diagnosing inter-class dependencies, and learned biases) and at the local level 
% (e.g., understanding misclassifications).

% In this work, we take an alternative approach for explaining deep networks. 
% At a high level, we first decompose a given deep network into 
% a deep representation followed by the final linear layer and instead focus on 
% the relatively simpler problem of interpreting the linear model. 
% Despite the linearity, this task can be highly non-trivial for typical modern deep networks, 
% whose final linear classifiers have up to thousands of (learned) input features 
% and millions of parameters. 
% To alleviate this problem, our strategy is to 
% optimally replace the \emph{dense} linear layer of a given deep 
% network with a \emph{sparse} one (cf. Figure~\ref{fig:decomposition}) which 
% maintains comparable performance. 
% We can then leverage the strengths of existing interpretability techniques: a 
% naturally interpretable linear model~\cite{studies} explains how the network 
% makes its decisions 
% based on a sparse set of features, which in turn, can be understood using 
% standard feature interpretation methods.  

% Although simple in concept, our approach allows us to develop a 
% deeper understanding of the internal reasoning process of complex 
% architectures. The resulting explanations can serve as a powerful 
% tool to debug state-of-the-art deep networks, both at the global level (e.g., 
% diagnosing inter-class dependencies, and learned biases) and at the local level 
% (e.g., understanding misclassifications).

% \paragraph{Our contributions.}
% \begin{itemize}
% 	\item The core tool, that forms the basis of our approach, is an optimized, GPU 
% 	accelerated solver for fitting regularized generalized linear models (GLMs) on 
% 	deep representations. This allows us to replace the dense linear layer of a 
% 	given deep network with a sparse, and thus interpretable one. Note that our 
% 	accelerated solver is key to doing so as both state-of-the-art 
% 	GLM solvers and standard backpropagation libraries simply cannot scale to 
% 	ImageNet-scale datasets. 
	
% 	\item We demonstrate that the final linear classifier 
% 	of standard deep networks can be greatly sparsified (by several orders of 
% 	magnitude) to depend on a small number of features using our GLM solver 
% 	on a variety of vision and text classification tasks. These 
% 	gains in sparsity for the linear classifier can be 
% 	obtained at a marginal cost to accuracy, and in some cases 
% 	actually improve accuracy. 

% 	% Eric: I still think we remove this part unless we actually do 
% 	% some experiments here. 
% 	% An added advantage of the GLM framework is that it can also be 
% 	% used to compute the relative-ordering of feature importance within 
% 	% the deep representation layer.
	
% 	\item Finally, we use our explanation to perform in-depth analysis of 
% 	state-of-the-art deep networks and demonstrate how they can be used to 
% 	identify (spurious) correlations, explain misclassifications, and uncover 
% 	biases learned from the data. 
% 	We complement our experiments with a human-in-the-loop evaluation of our 
% 	explanations using Amazon Turk.
% \end{itemize} 
%
%\shibani{Rather than saying this is an interpretability method, maybe a step 
%	towards making the interpretability problem more tractable. Specifically, you 
%	can reason about the model decisions in terms of a small set of features. 
%	Find references which use linear models for interpretability. Have been 
%	extensively studied. }
%\shibani{Random thoughts: i) gives you a dictionary to compare predictions 
%	between different samples/classes; ii) bring the advantages of sparse linear 
%	models to deep networks; iii) a way to step away from trade-offs between 
%	model faithfulness and complexity, (iv) not instance specific}

\begin{figure}[t]
	\includegraphics[width=\columnwidth]{figures/intro/overview}
	\caption{example caption}
	\label{fig:decomposition}
\end{figure}


%\eric{may need some reworking}
%In this paper, we leverage the complementary strengths of these two types 
%of approaches to instead study \emph{global} explanations of how a deep 
%network 
%makes predictions. 
%Our work builds upon feature interpretation methods by greatly reducing the 
%working set of features to a tractible size, which allows practitioners to 
%focus their attention and analyze only the features that matter most. 
%\shibani{This 
%is not true though?}
%In contrast to feature attribution methods, our explanations are 
%example-agnostic and capture the general reasoning process of the deep 
%network.

%\paragraph{contribution: using GLMs in tandem with network 
%interpretability tools to provide sparse network explanations for model 
%predictions}
%\paragraph{contribution: scaling the GLM to modern problems deep 
%learning problems}
%\paragraph{contribution: amazon turk experiments for measuring how 
%aligned our interpretability is with humans}
